Ten Years of ZMap

Since ZMap's debut in 2013, networking and security researchers have used the open-source scanner to write hundreds of research papers that study Internet behavior. In addition, ZMap has been adopted by the security industry to build new classes of enterprise security and compliance products. Over the past decade, much of ZMap's behavior -- ranging from its pseudorandom IP generation to its packet construction -- has evolved as we have learned more about how to scan the Internet. In this work, we quantify ZMap's adoption over the ten years since its release, describe its modern behavior (and the measurements that motivated changes), and offer lessons from releasing and maintaining ZMap for future tools.

==> zmap_shard_pizza.tex <==
\begin{tikzpicture}[
auto,                %
node distance = 0cm, %
]

\node[circle, draw=black, very thick, minimum size=5.cm] (center) at (0,0)  {};

\foreach \angle / \clr / \lab / \address in {%
90/blue/a0/$s_0$, 67.5/blue/a1/$s_1$, 45/blue/a2/$s_2$, 
22.5/blue/a3/$s_3$, 0/blue/a4/$s_4$, 337.5/blue/a5/$s_5$, 
315/green/a6/$s_6$, 292.5/green/a7/$s_7$, 270/green/a8/$s_8$,
247.5/green/a9/$s_9$, 225/green/a10/$s_{10}$,
202.5/orange/a11/$s_{11}$, 180/orange/a12/$s_{12}$, 157.5/orange/a13/$s_{13}$, 
135/orange/a14/$s_{14}$, 112.5/orange/a15/$s_{15}$
}
\draw (\angle:2.5cm) node [circle, draw=\clr, fill=white, very thick, minimum size=.8cm] (\lab) {\address};


\path[very thick,->,draw=blue] (a0) edge[bend right=90] node [left] {} (a1);
\path[very thick,->,draw=blue] (a1) edge[bend right=90] node [left] {} (a2);
\path[very thick,->,draw=blue] (a2) edge[bend right=90] node [left] {} (a3);
\path[very thick,->,draw=blue] (a3) edge[bend right=90] node [left] {} (a4);
\path[very thick,->,draw=blue] (a4) edge[bend right=90] node [left] {} (a5);

\path[very thick,->,draw=green] (a6) edge[bend right=90] node [left] {} (a7);
\path[very thick,->,draw=green] (a7) edge[bend right=90] node [left] {} (a8);
\path[very thick,->,draw=green] (a8) edge[bend right=90] node [left] {} (a9);
\path[very thick,->,draw=green] (a9) edge[bend right=90] node [left] {} (a10);

\path[very thick,->,draw=orange] (a11) edge[bend right=90] node [left] {} (a12);
\path[very thick,->,draw=orange] (a12) edge[bend right=90] node [left] {} (a13);
\path[very thick,->,draw=orange] (a13) edge[bend right=90] node [left] {} (a14);
\path[very thick,->,draw=orange] (a14) edge[bend right=90] node [left] {} (a15);


\node[text=blue] (shard0_label) [above left=-1.5cm and -2.cm of center] {Shard 0};
\node[text=green] (shard1_label) [below=0cm of shard0_label] {Shard 1};
\node[text=orange] (shard2_label) [below=0cm of shard1_label] {Shard 2};

\node[] (shard0_label_left) [right=-0.2cm of shard0_label] {};
\node[] (shard0_label_right) [right=0.6cm of shard0_label] {};
\path[very thick,->,draw=blue] (shard0_label_left) edge[right] node [left] {} (shard0_label_right);

\node[] (shard1_label_left) [right=-0.2cm of shard1_label] {};
\node[] (shard1_label_right) [right=0.6cm of shard1_label] {};
\path[very thick,->,draw=green] (shard1_label_left) edge[right] node [left] {} (shard1_label_right);

\node[] (shard2_label_left) [right=-0.2cm of shard2_label] {};
\node[] (shard2_label_right) [right=0.6cm of shard2_label] {};
\path[very thick,->,draw=orange] (shard2_label_left) edge[right] node [left] {} (shard2_label_right);

\end{tikzpicture}



==> zmap_shard_zippier.tex <==
\begin{tikzpicture}[
     auto,                %
     node distance = 0cm, %
  ]
  
  \node[circle, draw=black, very thick, minimum size=5.cm] (center) at (0,0)  {};
  
  \foreach \angle / \clr / \lab / \address in {%
    90/blue/a0/$s_0$, 67.5/green/a1/$s_1$, 45/orange/a2/$s_2$, 
    22.5/blue/a3/$s_3$, 0/green/a4/$s_4$, 337.5/orange/a5/$s_5$, 
    315/blue/a6/$s_6$, 292.5/green/a7/$s_7$, 270/orange/a8/$s_8$,
    247.5/blue/a9/$s_9$, 225/green/a10/$s_{10}$, 202.5/orange/a11/$s_{11}$,
    180/blue/a12/$s_{12}$, 157.5/green/a13/$s_{13}$, 135/orange/a14/$s_{14}$, 
    112.5/blue/a15/$s_{15}$
   }
    \draw (\angle:2.5cm) node [circle, draw=\clr, fill=white, very thick, minimum size=.8cm] (\lab) {\address};
    
    
  \path[very thick,->,draw=blue] (a0) edge[bend right] node [left] {} (a3);
  \path[very thick,->,draw=blue] (a3) edge[bend right] node [left] {} (a6);
  \path[very thick,->,draw=blue] (a6) edge[bend right] node [left] {} (a9);
  \path[very thick,->,draw=blue] (a9) edge[bend right] node [left] {} (a12);
  \path[very thick,->,draw=blue] (a12) edge[bend right] node [left] {} (a15);
    
  \path[very thick,->,draw=green] (a1) edge[bend right] node [left] {} (a4);
  \path[very thick,->,draw=green] (a4) edge[bend right] node [left] {} (a7);
  \path[very thick,->,draw=green] (a7) edge[bend right] node [left] {} (a10);
  \path[very thick,->,draw=green] (a10) edge[bend right] node [left] {} (a13);
  
  \path[very thick,->,draw=orange] (a2) edge[bend right] node [left] {} (a5);
  \path[very thick,->,draw=orange] (a5) edge[bend right] node [left] {} (a8);
  \path[very thick,->,draw=orange] (a8) edge[bend right] node [left] {} (a11);
  \path[very thick,->,draw=orange] (a11) edge[bend right] node [left] {} (a14);
    
     
  \node[text=blue] (shard0_label) [above left=-1.5cm and -2.cm of center] {Shard 0};
  \node[text=green] (shard1_label) [below=0cm of shard0_label] {Shard 1};
  \node[text=orange] (shard2_label) [below=0cm of shard1_label] {Shard 2};
  
  \node[] (shard0_label_left) [right=-0.2cm of shard0_label] {};
  \node[] (shard0_label_right) [right=0.6cm of shard0_label] {};
  \path[very thick,->,draw=blue] (shard0_label_left) edge[right] node [left] {} (shard0_label_right);
  
  \node[] (shard1_label_left) [right=-0.2cm of shard1_label] {};
  \node[] (shard1_label_right) [right=0.6cm of shard1_label] {};
  \path[very thick,->,draw=green] (shard1_label_left) edge[right] node [left] {} (shard1_label_right);
  
  \node[] (shard2_label_left) [right=-0.2cm of shard2_label] {};
  \node[] (shard2_label_right) [right=0.6cm of shard2_label] {};
  \path[very thick,->,draw=orange] (shard2_label_left) edge[right] node [left] {} (shard2_label_right);
  
  
  
  
\end{tikzpicture}

